User-Device Authentication in Mobile Banking using APHEN for Paratuck2 Tensor Decomposition

The new financial European regulations such as PSD2 are changing the retail banking services. Noticeably, the monitoring of the personal expenses is now opened to other institutions than retail banks. Nonetheless, the retail banks are looking to leverage the user-device authentication on the mobile banking applications to enhance the personal financial advertisement. To address the profiling of the authentication, we rely on tensor decomposition, a higher dimensional analogue of matrix decomposition. We use Paratuck2, which expresses a tensor as a multiplication of matrices and diagonal tensors, because of the imbalance between the number of users and devices. We highlight why Paratuck2 is more appropriate in this case than the popular CP tensor decomposition, which decomposes a tensor as a sum of rank-one tensors. However, the computation of Paratuck2 is computational intensive. We propose a new APproximate HEssian-based Newton resolution algorithm, APHEN, capable of solving Paratuck2 more accurately and faster than the other popular approaches based on alternating least square or gradient descent. The results of Paratuck2 are used for the predictions of users' authentication with neural networks. We apply our method for the concrete case of targeting clients for financial advertising campaigns based on the authentication events generated by mobile banking applications.

==> 2_Theory/bc_resolution.tex <==
\subsection{Other Popular Resolution Schemes}
Hereinafter, we describe three types of popular numerical for tensor resolution that are used to compare the convergence of our approach. 

\subsubsection{Gradient Free Resolution}
The Alternating Least Square (ALS) is a gradient-free numerical resolution introduced in \cite{harshman1970foundations,carroll1970analysis}. Following the description of the non-negative matrix multiplication update \cite{lee1999learning}, the non-negative scheme for the CP decomposition was introduced in \cite{welling2001positive}. Since it is a gradient-free method, it does not rely on any derivatives to find the optimal solution of the tensor error minimization problem underlined in \ref{eq::errorminimization}. It consists in an iterative update of the matrices $\textbf{A}, \textbf{H}$ and $\textbf{B}$ and the tensors $\mathscr{D}^A$ and $\mathscr{D}^B$. It fixes $\mathscr{D}^A, \textbf{H}, \mathscr{D}^B$ and $\textbf{B}$ to solve $\textbf{A}$. Then, it fixes $\textbf{A}, \textbf{H}, \mathscr{D}^B$ and $\textbf{B}$ to solve $\mathscr{D}^A$. The same methodology is used to solve the other factors. After the update of the matrix $\textbf{B}$, the process starts again repeating itself until some convergence criterion is satisfied. We present the complete ALS for Paratuck2 in the algorithm \ref{algo:nnals}.

\SetAlFnt{\footnotesize}
\SetAlCapFnt{\footnotesize}
\SetAlCapNameFnt{\footnotesize}

\begin{algorithm}[b!]
\setstretch{1.25}
\DontPrintSemicolon

\KwData{tensor $\mathscr{X} \in \mathbb{R}^{I\times J\times K}$, latent factors $(P,Q)$}

\KwResult{$\textbf{A}, \mathscr{D}^A, \textbf{H}, \mathscr{D}^B, \textbf{B}$ from tensor decomposition}

\Begin{

random initialization A$\in\mathbb{R}^{I\times P}$

random initialization H$\in\mathbb{R}^{P\times Q}$

random initialization B$\in\mathbb{R}^{J\times Q}$

set $\mathscr{D}^A_k \in\mathbb{R}^{P\times P}$ equal to 1 for $k=1,...,K$

set $\mathscr{D}^B_k \in\mathbb{R}^{Q\times Q}$ equal to 1 for $k=1,...,K$

$\textbf{X} = \left[ \textbf{X}_1 \: \textbf{X}_2 \cdots \textbf{X}_k \right]$

$\textbf{x} = \textrm{vec}(\mathscr{X})$

\Repeat{maximum number of iterations or stopping criteria}{
$a_{ip}\gets a_{ip} 
	\dfrac{\left[ \textbf{X} \textbf{F}^T\right]_{ip}}
	{\left[ \textbf{A}(\textbf{FF}^T) \right]_{ip}} 
	\:, \:
	\textbf{F}=\mathscr{D}^A \textbf{H}\mathscr{D}^B \textbf{B}^T$
    
$d^a_{pp}\gets d^a_{pp}
	\dfrac{\left[ \textbf{Z}^T \textbf{x} \right]_{pp}}
	{\left[ \mathscr{D}^A(\textbf{ZZ}^T) \right]_{pp}} 
	\:, \:
	\textbf{Z}=(\textbf{B}\mathscr{D}^B \textbf{H}^T) \odot\textbf{A}$
    
$h_{pq}\gets h_{pq}
	\dfrac{\left[ \textbf{Z}^T \textbf{x} \right]_{pq}}
	{\left[ \textbf{H}(\textbf{ZZ}^T) \right]_{pq}} 
	\:, \:
	\textbf{Z}=\textbf{B} \mathscr{D}^B \otimes \textbf{A} \mathscr{D}^A$
    
$d^b_{qq}\gets d^b_{qq}
	\dfrac{\left[ \textbf{x} \textbf{Z} \right]_{qq}}
	{\left[ \mathscr{D}^B (\textbf{Z}^T\textbf{Z})\right]_{qq}}
	\:, \:
	\textbf{Z}=\textbf{B} \odot (\textbf{H}^T \mathscr{D}^A\textbf{A}^T)^T$
    
$b_{qj}\gets b_{qj} 
	\dfrac{\left[ \textbf{X}^T \textbf{F}^T \right]_{qj}}
	{\left[ \textbf{B}(\textbf{F} \textbf{F}^T) \right]_{qj}} 
	\:, \:
	\textbf{F}= (\textbf{A} \mathscr{D}^A \textbf{H}\mathscr{D}^B)^T$

}
\KwRet{$\textbf{A}, \mathscr{D}^A, \textbf{H}, \mathscr{D}^B, \textbf{B}$}
}

\caption{Non-negative ALS algorithm applied to Paratuck2 decomposition for a tensor $\mathscr{X}$ of size $\mathbb{R}^{I\times J\times K}$ of latent factors $(P,Q)$\label{algo:nnals}}
\end{algorithm}


\subsubsection{Hessian Free Resolution}
The gradient descent method, or Hessian-free method, operates solely on the first derivative to solve the error minimization problem. Hereinafter, we describe four of the most renown gradient-based methods: the standard Gradient Descent (GD) update, the Nesterov Accelerated Gradient (NAG), Adam and SAGA. We present the gradient descent scheme with the standard gradient update. Then, we simply describe the update of the optimal solution.

In the gradient descent method applied to error minimization, the minimization function decreases the fastest in opposite direction of the gradient. Therefore, the error is reduced through an iterative procedure. At each iteration, the current solution is subtracted by its gradient for a small step size. In the standard gradient descent update, the step size of the descent is fixed small enough to ensure the convergence of he iterations. The update of the optimal solution of the error minimization function at iteration $n$ follows equation \ref{eq::gradesc}
\begin{equation}
\label{eq::gradesc}
\textbf{x}_{n+1} = \textbf{x}_n - \gamma_n \nabla f(\textbf{x}_n)
\end{equation}
with $\gamma_n$ the variable step size and $\nabla f$ the gradient of $f$ according to equation \ref{eq::gradient}. Some implementations use a fixed step size $\gamma$. However, to improve the convergence of the gradient scheme, we compute a variable step size $\gamma_n$ using the Wolfe's line search. The algorithm is shown in \ref{algo:gradesc}.


The Nesterov Accelerated Gradient (NAG) is a solution to increase the convergence of the gradient descent iterative process. Instead of using the equation \ref{eq::gradesc}, the update of the optimal solution is described by 
\begin{equation}
\label{eq::nesterov}
\begin{cases}
\textbf{v}_n = \gamma \textbf{v}_{n-1}
+ \eta \nabla f(\textbf{x}_n-\gamma \textbf{v}_{n-1})\\
\textbf{x}_{n+1} = \textbf{x}_n -\textbf{v}_n
\end{cases}
\end{equation}
with $\gamma = 0.9$ and $\eta=0.001$. NAG is designed to approximate the next position relying on the velocity denoted by $v$.

The Adam, or Adaptive Moment Estimation, update rule is one of the most popular scheme in machine learning nowadays. It evaluates adaptive learning rates for the velocity, $v_t$, and the momentum, $m_t$. Adam stores an exponentially decaying average of past gradients and past squared gradients
\begin{equation}
\label{eq::adam}
\begin{cases}
\textbf{m}_n = \beta_1 \textbf{m}_{n-1} + (1-\beta_1) \nabla f(\textbf{x}_n) \\
\textbf{v}_n = \beta_2 \textbf{v}_{n-1} + (1-\beta_2) (\nabla f(\textbf{x}_n))^2 \\
\widehat{\textbf{m}}_n = \dfrac{\textbf{m}_n}{1-\beta_1} \\
\widehat{\textbf{v}}_n = \dfrac{\textbf{v}_n}{1-\beta_2} \\
\textbf{x}_{n+1} = \textbf{x}_n - \dfrac{\eta}{\sqrt{\widehat{\textbf{v}}_n}+\epsilon}\widehat{\textbf{m}}_n
\end{cases}
\end{equation}
with $\beta_1=0.9$, $\beta_2=0.999$, $\epsilon=10^{-8}$ and $\eta=0.001$ determined experimentally in \cite{kingma2014adam}.

Finally, SAGA is the last update for the gradient descent method we present in our paper. This update stores the gradient during the calculation. The current gradient, the past gradient and the mean of the past gradient are used for the update as described in \cite{defazio2014saga}.
\begin{equation}
\label{eq::saga}
\textbf{x}_{n+1} = \textbf{x}_n - \gamma_n \left( \nabla f(\textbf{x}_n) - \nabla f(\textbf{x}_{n-1}) + \dfrac{1}{n} \sum_{i=1}^n \nabla f(\textbf{x}_{n-1}^{(i)}) \right)
\end{equation}
The term $\gamma_n$ is a variable step size determined with the Wolfe's line search and $\textbf{x}_{n-1}^{(i)}$ the \textit{i}-th element of the vector $\textbf{x}$ of the $n-1$ iteration.

Nonetheless, Hessian-free methods are very sensitive to local minima. The initial guess of the optimal solution is determinant to ensure global convergence at the end of the minimization process. Therefore, Hessian-based methods have been introduced to overcome local minima issues.


%
%
%
% ==========================
%     NEW SUBSUBSECTION
% ==========================
\subsubsection{Resolution with Hessian Approximation}
The BFGS method has been simultaneously introduced in \cite{broyden1970convergence, fletcher1970new, goldfarb1970family, shanno1970conditioning}. It uses the Hessian matrix for a faster convergence but does not evaluate directly the Hessian matrix. We only highlight the difference in the Hessian computation since it is the major difference with ApHeN presented in the algorithm \ref{algo:newcg}. At each iteration, the matrix $\textbf{B}$, replacing the Hessian matrix denoted previously by $\textbf{Hes}$, is evaluated with the descent direction $\textbf{p}_n$, the step size $\alpha_n$ and the gradient evolution. The calculation of $\textbf{B}$ follows the system of equation \ref{eq::bfgs}.
\begin{equation}
\label{eq::bfgs}
\begin{cases}
\textbf{s}_n = \alpha_n \textbf{p}_n \\
\textbf{y}_n = \nabla f(\textbf{x}_{n+1}) - \nabla f(\textbf{x}_n) \\
\textbf{B}_{n+1} = \textbf{B}_n + \dfrac{\textbf{y}_n\textbf{y}_n^T}{\textbf{y}_n^T\textbf{s}_n} - \dfrac{\textbf{B}_n\textbf{s}_n\textbf{s}_n^T\textbf{B}_n}{\textbf{s}_n^T\textbf{B}_n\textbf{s}_n}
\end{cases}
\end{equation}
At the initial step, the matrix $\textbf{B}_0$ can be initialized such that $\textbf{B}_0$ equals the identity matrix. More information about the implementation of the algorithm can be found in \cite{wright1999numerical}.


\SetAlFnt{\footnotesize}
\SetAlCapFnt{\footnotesize}
\SetAlCapNameFnt{\footnotesize}

\begin{algorithm}[b!]
\setstretch{1.25}
\DontPrintSemicolon

\KwData{tensor $\mathscr{X} \in \mathbb{R}^{I\times J\times K}$, latent factors $(P,Q)$}

\KwResult{$\textbf{A}, \mathscr{D}^A, \textbf{H}, \mathscr{D}^B, \textbf{B}$ from tensor decomposition}

\Begin{

random initialization A$\in\mathbb{R}^{I\times P}$

random initialization H$\in\mathbb{R}^{P\times Q}$

random initialization B$\in\mathbb{R}^{J\times Q}$

set $\mathscr{D}^A_k \in\mathbb{R}^{P\times P}$ equal to 1 for $k=1,...,K$

set $\mathscr{D}^B_k \in\mathbb{R}^{Q\times Q}$ equal to 1 for $k=1,...,K$

\textbf{x}$_0$ $\gets$ flatten($\textbf{A}$, $\mathscr{D}^A$, $\textbf{H}$, $\mathscr{D}^B$, $\textbf{B}$) as described in (\ref{eq::vectorize_x})

\Switch{Gradient Descent \textbf{or} NAG \textbf{or} Adam \textbf{or} SAGA}{
initialized fixed parameters of \ref{eq::gradesc} or \ref{eq::nesterov} or \ref{eq::adam} or \ref{eq::saga}
}

$n = 0$

\Repeat{maximum number of iterations or stopping criteria}{

$\nabla \textit{f}_n = \dfrac{\partial}{\partial x_i} f(\textbf{x}_n)$ $\gets$ gradient of $f$ at $\textbf{x}_n$ with (\ref{eq::fourth_order_diff})

\Switch{Gradient Descent \textbf{or} NAG \textbf{or} Adam \textbf{or} SAGA}{
update $\textbf{x}_{n+1}$ with \ref{eq::gradesc} or \ref{eq::nesterov} or \ref{eq::adam} or \ref{eq::saga}
}

$n = n +1$

}
\KwRet{$\textbf{A}, \mathscr{D}^A, \textbf{H}, \mathscr{D}^B, \textbf{B}$}
}

\caption{Gradient descent algorithm applied to Paratuck2 decomposition for a tensor $\mathscr{X}\in\mathbb{R}^{I\times J\times K}$ of latent factors $(P, Q)$\label{algo:gradesc}}
\end{algorithm}









